On the Achievable Rates of Decentralized Equalization in Massive MU-MIMO Systems

Massive multi-user (MU) multiple-input multiple-output (MIMO) promises significant gains in spectral efficiency compared to traditional, small-scale MIMO technology. Linear equalization algorithms, such as zero forcing (ZF) or minimum mean-square error (MMSE)-based methods, typically rely on centralized processing at the base station (BS), which results in (i) excessively high interconnect and chip input/output data rates, and (ii) high computational complexity. In this paper, we investigate the achievable rates of decentralized equalization that mitigates both of these issues. We consider two distinct BS architectures that partition the antenna array into clusters, each associated with independent radio-frequency chains and signal processing hardware, and the results of each cluster are fused in a feedforward network. For both architectures, we consider ZF, MMSE, and a novel, non-linear equalization algorithm that builds upon approximate message passing (AMP), and we theoretically analyze the achievable rates of these methods. Our results demonstrate that decentralized equalization with our AMP-based methods incurs no or only a negligible loss in terms of achievable rates compared to that of centralized solutions.

==> macros/delta_star.tex <==
% This file was created by matlab2tikz v0.4.7 running on MATLAB 8.1.
% Copyright (c) 2008--2014, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% Minimal pgfplots version: 1.3
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
\begin{tikzpicture}

\begin{axis}[%
width=5.16317052165354in,
height=3.59478807824803in,
scale only axis,
xmin=0.5,
xmax=1,
xlabel={$\sigma{}^\text{2}$},
xmajorgrids,
ymin=-0.1,
ymax=0.02,
ylabel={$\text{MSE }\Psi\text{(}\sigma{}^\text{2}\text{,}\delta\text{)}$},
ymajorgrids,
legend style={draw=black,fill=white,legend cell align=left},
scaled y ticks = false,
y tick label style={/pgf/number format/.cd, fixed, fixed zerofill,precision=2}
]
\addplot [color=blue,solid,line width=2.0pt]
  table[row sep=crcr]{0.5	-0.00847186823552865\\
0.51	-0.00601453905159377\\
0.52	-0.00370544732742462\\
0.53	-0.00154476341156906\\
0.54	0.000467627376738888\\
0.55	0.00233209087222286\\
0.56	0.00404921374335487\\
0.57	0.0056197763556024\\
0.58	0.0070447284855838\\
0.59	0.00832516758867108\\
0.6	0.00946231935404707\\
0.61	0.010457520309356\\
0.62	0.0113122022622594\\
0.63	0.0120278783886857\\
0.64	0.0126061307976336\\
0.65	0.0130485994203295\\
0.66	0.0133569720875105\\
0.67	0.0135329756729161\\
0.68	0.0135783681937844\\
0.69	0.0134949317705579\\
0.7	0.0132844663581388\\
0.71	0.0129487841701174\\
0.72	0.0124897047255125\\
0.73	0.0119090504547793\\
0.74	0.0112086428083547\\
0.75	0.0103902988167651\\
0.76	0.00945582805653367\\
0.77	0.0084070299807415\\
0.78	0.00724569157726995\\
0.79	0.00597358532146186\\
0.8	0.0045924673932799\\
0.81	0.003104076132037\\
0.82	0.00151013070445061\\
0.83	-0.000187670035805887\\
0.84	-0.00198764851672595\\
0.85	-0.0038881492624897\\
0.86	-0.00588753956984844\\
0.87	-0.00798421006078442\\
0.88	-0.0101765751244192\\
0.89	-0.0124630732598896\\
0.9	-0.0148421673307546\\
0.91	-0.0173123447404596\\
0.92	-0.0198721175374564\\
0.93	-0.0225200224577413\\
0.94	-0.0252546209118061\\
0.95	-0.0280744989223199\\
0.96	-0.0309782670182411\\
0.97	-0.0339645600904978\\
0.98	-0.037032037213876\\
0.99	-0.0401793814392991\\
1	-0.0434052995602611\\
};
\addlegendentry{$\delta\text{=0.48}$};

\addplot [color=black!50!green,solid,line width=2.0pt]
  table[row sep=crcr]{0.5	-0.0187120376472885\\
0.51	-0.0165142361546856\\
0.52	-0.0144615838414366\\
0.53	-0.0125542475071614\\
0.54	-0.0107921148602765\\
0.55	-0.00917482768761513\\
0.56	-0.00770181154296512\\
0.57	-0.00637230231847263\\
0.58	-0.00518537002453257\\
0.59	-0.00413994006942631\\
0.6	-0.00323481229916234\\
0.61	-0.00246867803042228\\
0.62	-0.00184013528487104\\
0.63	-0.00134770241107862\\
0.64	-0.00098983026065036\\
0.65	-0.000764913067593964\\
0.66	-0.000671298164312661\\
0.67	-0.000707294653602974\\
0.68	-0.000871181143586086\\
0.69	-0.00116121264132862\\
0.7	-0.0015756266909891\\
0.71	-0.00211264883342677\\
0.72	-0.00277049745626901\\
0.73	-0.0035473880963619\\
0.74	-0.00444153725015284\\
0.75	-0.00545116574191751\\
0.76	-0.00657450169464413\\
0.77	-0.00780978314385727\\
0.78	-0.00915526033058989\\
0.79	-0.0106091977060686\\
0.8	-0.0121698756774135\\
0.81	-0.0138355921207137\\
0.82	-0.0156046636852255\\
0.83	-0.01747542691006\\
0.84	-0.0194462391726276\\
0.85	-0.0215154794861878\\
0.86	-0.0236815491621433\\
0.87	-0.0259428723511849\\
0.88	-0.0282978964759938\\
0.89	-0.0307450925669753\\
0.9	-0.0332829555113638\\
0.91	-0.0359100042250333\\
0.92	-0.0386247817554261\\
0.93	-0.0414258553232051\\
0.94	-0.0443118163094768\\
0.95	-0.0472812801947716\\
0.96	-0.050332886455361\\
0.97	-0.0534652984219457\\
0.98	-0.0566772031052537\\
0.99	-0.0599673109926471\\
1	-0.0633343558194223\\
};
\addlegendentry{$\delta\text{=0.49}$};

\addplot [color=red,solid,line width=2.0pt]
  table[row sep=crcr]{0.5	-0.0285342409606091\\
0.51	-0.0265853741923451\\
0.52	-0.0247786943752848\\
0.53	-0.0231143649049744\\
0.54	-0.0215922757814954\\
0.55	-0.0202120761021536\\
0.56	-0.0189732031441291\\
0.57	-0.0178749083936059\\
0.58	-0.0169162808403585\\
0.59	-0.0160962678231115\\
0.6	-0.015413693680812\\
0.61	-0.0148672764379647\\
0.62	-0.0144556427280369\\
0.63	-0.0141773411373831\\
0.64	-0.0140308541328821\\
0.65	-0.0140146087192757\\
0.66	-0.0141269859568777\\
0.67	-0.0143663294565907\\
0.68	-0.0147309529569823\\
0.69	-0.0152191470772199\\
0.7	-0.0158291853299485\\
0.71	-0.0165593294694794\\
0.72	-0.0174078342428757\\
0.73	-0.0183729516045994\\
0.74	-0.0194529344491293\\
0.75	-0.0206460399104498\\
0.76	-0.0219505322723045\\
0.77	-0.0233646855286765\\
0.78	-0.0248867856299656\\
0.79	-0.0265151324467612\\
0.8	-0.0282480414799152\\
0.81	-0.03008384534274\\
0.82	-0.0320208950385883\\
0.83	-0.0340575610547527\\
0.84	-0.0361922342915535\\
0.85	-0.0384233268436126\\
0.86	-0.0407492726486302\\
0.87	-0.0431685280174872\\
0.88	-0.0456795720581163\\
0.89	-0.0482809070043839\\
0.9	-0.0509710584601116\\
0.91	-0.0537485755673797\\
0.92	-0.0566120311073562\\
0.93	-0.0595600215410989\\
0.94	-0.0625911669970385\\
0.95	-0.0657041112112049\\
0.96	-0.0688975214256599\\
0.97	-0.0721700882500693\\
0.98	-0.0755205254908607\\
0.99	-0.0789475699519808\\
1	-0.0824499812108627\\
};
\addlegendentry{$\delta\text{=0.50}$};

\end{axis}
\end{tikzpicture}%
